Randomized Gossiping with Effective Resistance Weights: Performance Guarantees and Applications

The effective resistance between a pair of nodes in a weighted undirected graph is defined as the potential difference induced when a unit current is injected at one node and extracted from the other, treating edge weights as the conductance values of edges. The effective resistance is a key quantity of interest in many applications, e.g., solving linear systems, Markov Chains, and continuous-time averaging networks. We consider effective resistances (ER) in the context of designing randomized gossiping methods for the consensus problem, where the aim is to compute the average of node values in a distributed manner through iteratively computing weighted averages among randomly chosen neighbors. We show that employing ER weights improves the averaging time corresponding to the traditional choice of uniform weights -the amount of improvement depends on the network structure. We illustrate these results through numerical experiments. We also present an application of the ER gossiping to distributed optimization: we numerically verified that using ER gossiping within EXTRA and DPGA-W methods improves their practical performance in terms of communication efficiency.

==> Methodology.tex <==
%\vspace{-2mm}
\section{Distributed Computation of Effective Resistances}\label{sec-method}
\bc{Section \ref{sec-theoretical guarantees} proves that using effective resistance-based probabilities in consensus improves the $\varepsilon$-averaging time performance of the algorithms on $c$-barbell graphs and graphs with a diameter $\mathcal{D}$.In this section, we change our focus from analysis of $\mathcal{A}(P^r)$ to computation of these weights on agents. Best to our knowledge, distributed computation of effective resistances over graphs is first appeared in in \cite{aybat2017decentralized}. Aybat et al proposed a variation of distributed randamized Kaczmarz method (D-RK) to solve this computation problem. First, we briefly summarise the work of Aybat et al in \cite{aybat2017decentralized} for the sake of completeness and then provide the linear convergence of the proposed algorithm.
Remember that effective resistance $R_{ij}$ between nodes $i$ and $j$ satisfy the identity 
$$
R_{ij}=\cL^{\dag}_{ii}+\cL^{\dag}_{jj}-2\cL_{ij}^{\dag},
$$ where $\cL^{\dag}$ is the pseudo inverse the Laplacian $\cL$ of the graph $\cG$. Hence, the distributed Kaczmarz method to compute $\cL^{\dag}$ in the next section solves the problem of distributed computation of effective resistance weights.}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Distributed Kaczmarz method for computing $\cL^\dag$:}
\label{sec:RK}
% Consider a \emph{consistent} linear system $Ax=b$, where $A=[a_i^\top]_{i=1}^m\in\reals^{m\times n}$ and $b\in\reals^m$. Suppose $A$ has no rows with all zeros, and let $x^*=\argmin\{\norm{x}_2:\ Ax=b\}$. In~\cite{gower2015stochastic}, it is shown that $x^*$ can be computed using a randomized %version of
% Kaczmarz method. %where the projections are computed according to a randomized order. Next, we briefly summarize the result in~\cite{gower2015stochastic}. More generally,
% In particular, it follows from the results in~\cite{gower2015stochastic} that starting from $x^0\in\N(A)$, the method displayed in Algorithm~\ref{alg:RK} produces $\{x^k\}_{k\geq 1}$ such that $\mathbb{E}[\norm{x^k-x^*}_2^2]\leq \rho^k\norm{x^0-x^*}_2^2$ for $k\geq 0$ with $\rho\triangleq 1-\lambda_{\min}^+(A^\top H A)$ {where $\lambda_{\min}^+(\cdot)$ denotes the smallest positive eigenvalue} and $H=\sum_{i=1}^mp_i \frac{1}{\norm{a_i}_2^2}e_ie_i^\top$; furthermore, $1-\frac{1}{\textbf{Rank}(A)}\leq \rho <1$. Note that fixing $p_i=\norm{a_i}_2^2/\norm{A}_F^2$ gives us the randomized Kaczmarz in~{\cite{strohmer2009randomized,zouzias2013randomized}}.%\vspace*{-3mm}

\bc{
It is well known that $\cL^{\dag}$ is the unique solution to the problem 
% $\cL\cL^\dag=\sum_{i=2}^nu_i u_i^\top$ and $\id=\sum_{i=1}^nu_i u_i^\top$; hence, $\cL\cL^\dag=\id-u_1u_1^\top=\id-\frac{1}{n}\one\one^\top$. Although {the solution set} $\{X\in\sym^n: \cL X=\id-\frac{1}{n}\one\one^\top\}$ has infinitely many elements, it is {well-known} that $\cL^\dag$ is the unique solution to
% %\vspace{-0.2pc}%the following problem:
\begin{align}
\label{eq:least-norm-system}
\cL^\dag=\argmin_{X\in\sym^n}\{\norm{X}_F:\ \cL X=B\},
%\vspace*{-5mm}
\end{align}
where $B\triangleq\id-\frac{1}{n}\one\one^\top$. Let $x^l, b^l\in\reals^n$ for $l\in\cN$ {be column vectors} such that $X=[x^l]_{l\in\cN}$ and $B=[b^l]_{l\in\cN}$, i.e., $b^l=e_l-\frac{1}{n}\one$. Note $n$ columns of $\cL^\dag$ can be computed in parallel:
%\vspace{-0.3pc}
{\begin{align}
\label{eq:projection}
x^l_*\triangleq\argmin_{x\in\reals^n}\{\norm{x}_2:\ \cL x= b^l\},\quad l\in\cN, %\vspace*{-8mm}
\end{align}}
i.e., $\cL^\dag=[x^l_*]_{l\in\cN}$. {%In fact,
Since $\cL^\dag\one=\zero$, %we have
$x^n_*=-\sum_{l=1}^{n-1}x^l_*$. Thus, one does not need to solve for all $l\in\cN$; it suffices to compute $\{x^l_*\}_{l\in\cN\setminus\{n\}}$ and calculate $x^n_*$ from these.
%one does not need to solve for all $l\in\cN$ since $\cL^\dag\one=\zero$; in particular, computing $\{x^l_*\}_{l\in\cN\setminus\{n\}}$ would be sufficient as $x^n_*=-\sum_{l=1}^{n-1}x^l_*$.
% Consider a \emph{consistent} linear system $Ax=b$, where $A=[a_i^\top]_{i=1}^m\in\reals^{m\times n}$ and $b\in\reals^m$. Suppose $A$ has no rows with all zeros, and let $x^*=\argmin\{\norm{x}_2:\ Ax=b\}$. 
In~\cite{gower2015stochastic}, it is shown that $x_*^{l}$ for all $l\in \cN$ can be computed using a randomized %version of
Kaczmarz method. 
In particular, it follows from the results in~\cite{gower2015stochastic} that starting from $x^{l,0}\in\N(A)$, the method displayed in Algorithm~\ref{alg:RK} produces $\{x^{l,k}\}_{k\geq 1}$ such that $\mathbb{E}[\norm{x^{l,k}-x_*^{l}}_2^2]\leq \rho^k\norm{x^{l,0}-x^*}_2^2$ for $k\geq 0$ with $\rho\triangleq 1-\lambda_{\min}^+(A^\top H A)$ {where $\lambda_{\min}^+(\cdot)$ denotes the smallest positive eigenvalue} and $H=\sum_{i=1}^mp_i \frac{1}{\norm{a_i}_2^2}e_ie_i^\top$; furthermore, $1-\frac{1}{\textbf{Rank}(A)}\leq \rho <1$. Note that fixing $p_i=\norm{a_i}_2^2/\norm{A}_F^2$ gives us the randomized Kaczmarz in~{\cite{strohmer2009randomized,zouzias2013randomized}}.%\vspace*{-3mm}
}
}
% Let $\{x^{l,k}\}_{k\geq 1}$ be the sequence generated when RK implemented on \eqref{eq:projection} for $l\in%\cN\setminus\{n\}
% \{1,\ldots,n-1\}$.
\DontPrintSemicolon
\begin{algorithm}
\small
\textbf{Initialization:} $x^{0}\in\N(A)$ \;
\For{$k\geq 0$}{
Pick $i\in\{1,\ldots,m\}$ with probability (w.p) $p_i$\;
$x^{k+1}\gets x^{k}-\frac{1}{\norm{a_i}^2}(a_i^\top x^{k}-b_i)a_i$\;
}
%\Return{$[\vartheta_i]_{i\in\cN}$}\;
\caption{\small RK($\{p_i\}_{i=1}^m$) -- Randomized Kaczmarz}
\label{alg:RK}
\end{algorithm}


In Algorithm~\ref{alg:step}, %{(Decentralized RK)}, %which we abbreviate by D-RK),
the distributed nature of RK steps are summarized assuming that each $i\in\cN$ has an exponential clock with rate $r_i>0$, and when its clock ticks, the node $i$ wakes up {and} communicates with its neighbors $j\in\cN_i$ on $\cG$. More precisely, consider the resulting superposition of these point processes, and let $\{t_k\}_{k\in\integers_+}$ be the times such that one of the clocks ticks; hence, for all $k\geq 0$, the node that wakes up at time $t_k$ is node $i$ with probability $p_i=r_i/\sum_{j\in\cN}r_i$, i.e., $\{t_k\}_{k\geq 0}$ denotes the arrival times of a Poisson process with rate $\sum_{j\in\cN}r_j$. %\vspace*{-2mm}
%Now fix $k\geq 1$ and suppose that at time $t_k$, $i$ wakes up and initiates Step$(k,i)$ as in Algorithm~\ref{alg:step} based on Algorithm~\ref{alg:RK}:
\DontPrintSemicolon
%\vspace{-2mm}
\begin{algorithm}
{\small
\textbf{Initialization:} $x_i^{l,0}\gets 0$ for $l\in\cN\setminus\{n\}$ and $i\in\cN$\;
\For{$k\geq 0$}{
At time $t_k$, $i\in\cN$ wakes up w.p. $p_i=\frac{r_i}{\sum_{j\in\cN}r_i}$\;
\For{$l\in%\cN\setminus\{n\}
\{1,\ldots,n-1\}$}{
Node $i$ requests and receives $x_j^{l,k}$ from $j\in\cN_i$\;
Node $i$ computes and sends $q_i^{l,k}$ to all $j\in\cN_i$
$q_i^{l,k}=\frac{1}{\sum_{j\in\cN_i\cup\{i\}}\cL_{ij}^2}(\sum_{j\in\cN_i\cup\{i\}}\cL_{ij}x^{l,k}_j-b^l_i)$\;
Each $j\in\cN_i\cup\{i\}$ updates $x_j^{l,k+1}\gets x_j^{l,k}-\cL_{ij}q_i^{l,k}$
}}}
\caption{\label{alg-drk}\small D-RK$(\{r_i\}_{i\in\cN})$ -- Decentralized RK}
\label{alg:step}
\end{algorithm}
%\vspace*{-2mm} 

For $k\geq 0$, let $X^k\triangleq [x^{l,k}]_{l\in\cN}$ be the concatenation of D-RK sequence, where $x^{n,k}\triangleq -\sum_{l=1}^{n-1}x^{l,k}$, and define 
    \BEQ\label{def-S} S=\diag(s) \quad \mbox{where} \quad s_i\triangleq\sum_{j\in\cN_i\cup\{i\}}\cL_{ij}^2 \mbox{ for } i\in\cN.
    \EEQ 
According to \cite{gower2015stochastic,strohmer2009randomized}, for $r_i=s_i$, we get $H=\frac{1}{\norm{\cL}_F^2}\id$, and this implies linear convergence of $\{X^k\}_{k\geq 0}$ to $\cL^\dag$ with rate 
\BEQ\label{def-rho}
\rho \triangleq 1-\left(\frac{\lambda_{\min}^+(\cL)}{\norm{\cL}_F}\right)^2,
\EEQ
i.e., $\mathbb{E}[\norm{X^k-\cL^\dag}_F^2]\leq \rho^k\norm{\cL^\dag}_F^2$ for $k\geq 0$. Moreover, for each $i\in\cN$, when node $i$ wakes up, Decentralized Randomized Kaczmarz (D-RK) defined by Algorithm \ref{alg-drk} requires $2d_i (n-1)$ communications -- each communication $i$ sends/receives a real variable to/from a neighboring node in $\cN_i$; hence, at each iteration, i.e., at each time a node wakes up, the expected number of communication per iteration is $N=\sum_{i\in\cN}2 p_i d_i (n-1)\leq 2d_{\max}(n-1)$. In particular, for unweighted graphs, i.e., $w_{ij}=1$ for $(i,j)\in\cE$, we have $p_i=\frac{d_i(d_i+1)}{2m+\sum_{j\in\cN}d_j^2}$ for $i\in\cN$.

Instead of \eqref{eq:least-norm-system}, consider implementing D-RK on a normalized system $S^{-\sfrac{1}{2}}\cL X = S^{-\sfrac{1}{2}} B$ to obtain better convergence rate in practice -- $i$-th equation in this normalized system can be computed locally at $i\in\cN$. For this system, where all the rows have unit norm, one can set $r_i=r$ for some $r>0$ for all $i\in\cN$ -- hence, nodes wake up with uniform probability, i.e., $p_i=\frac{1}{n}$ for $i\in\cN$; for this choice of equal clock rates, $H=\frac{1}{n}\id$ and $\{X^k\}_k$ converges linearly to $\cL^\dag$ with rate \BEQ\label{def-rhoS}{\rho_S} \triangleq 1-\frac{1}{n}\lambda_{\min}^{+}(\cL S^{-1}\cL).\EEQ 
Moreover, the expected number of communication per iteration is $N=4m\frac{n-1}{n}\leq 4m$. 
\bc{The following proposition is conjectured at \cite{aybat2017decentralized} by Aybat et al. We showed that such inequality is indeed valid for any type of graph, which implies that the normalized system is faster than $D-RK$. We deferred the proof of the proposition to Appendix} \ref{appendix-rate-compare}.
\begin{proposition}\label{prop-rate-compare} It holds that
{\small
\begin{equation}\frac{1}{n}\lambda_{\min}^+ (\cL S^{-1} \cL) \geq \left(\frac{\lambda_{\min}^+ (\cL)}{\| \cL\|_F}\right)^2,
\label{ineq-lambda-min-plus}
\end{equation}}%
where $S$ is given by \eqref{def-S}. Then, it follows that $\rho_S \leq \rho$ where $\rho$ and $\rho_S$ are defined by \eqref{def-rho} and \eqref{def-rhoS}. 
\end{proposition}

 
